J-MAC: Japanese multi-speaker audiobook corpus for speech synthesis

In this paper, we construct a Japanese audiobook speech corpus called "J-MAC" for speech synthesis research. With the success of reading-style speech synthesis, the research target is shifting to tasks that use complicated contexts. Audiobook speech synthesis is a good example that requires cross-sentence, expressiveness, etc. Unlike reading-style speech, speaker-specific expressiveness in audiobook speech also becomes the context. To enhance this research, we propose a method of constructing a corpus from audiobooks read by professional speakers. From many audiobooks and their texts, our method can automatically extract and refine the data without any language dependency. Specifically, we use vocal-instrumental separation to extract clean data, connectionist temporal classification to roughly align text and audio, and voice activity detection to refine the alignment. J-MAC is open-sourced in our project page. We also conduct audiobook speech synthesis evaluations, and the results give insights into audiobook speech synthesis.

==> fig/partitioning.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp3796101352946567] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (69.92,37.88) -- (329.92,37.88) -- (329.92,49.88) -- (69.92,49.88) -- cycle ;
%Shape: Rectangle [id:dp4918154254803251] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.54 ] (69.92,66.88) -- (170.92,66.88) -- (170.92,76.88) -- (69.92,76.88) -- cycle ;
%Shape: Rectangle [id:dp1263454580490353] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.56 ] (149.92,76.88) -- (260.92,76.88) -- (260.92,86.88) -- (149.92,86.88) -- cycle ;
%Shape: Rectangle [id:dp8775963547119923] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.55 ] (240.92,86.88) -- (329.92,86.88) -- (329.92,96.88) -- (240.92,96.88) -- cycle ;
%Straight Lines [id:da7856899965101948] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (69.92,27.88) -- (69.92,114.88) ;
%Straight Lines [id:da33561458894717244] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (160.92,44.88) -- (160.92,114.88) ;
%Straight Lines [id:da5346896577295797] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (250.92,43.88) -- (250.92,114.88) ;
%Straight Lines [id:da5540802931101504] 
\draw    (71.92,104.88) -- (158.92,104.88) ;
\draw [shift={(160.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(69.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15822088877530105] 
\draw    (253.92,104.88) -- (328.92,104.88) ;
\draw [shift={(330.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(251.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da653467356994818] 
\draw    (162.92,104.88) -- (249.92,104.88) ;
\draw [shift={(251.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(160.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21017878435256443] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (329.92,27.88) -- (329.92,114.88) ;
%Straight Lines [id:da640194301012043] 
\draw    (213.92,29.88) -- (327.92,29.88) ;
\draw [shift={(329.92,29.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da33763840313286453] 
\draw    (177.92,28.88) -- (71.92,28.88) ;
\draw [shift={(69.92,28.88)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da24706518655532705] 
\draw    (255.92,68.88) .. controls (256.88,49.58) and (266.23,56.36) .. (283.06,59.55) ;
\draw [shift={(284.92,59.88)}, rotate = 189.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10966678071540714] 
\draw    (250,69) -- (260.92,68.88) ;
\draw [shift={(260.92,68.88)}, rotate = 539.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;

% Text Node
\draw (104,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (281,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{last}}$};
% Text Node
\draw (194,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (187,20) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{full}}$};
% Text Node
\draw (286,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{overlap}}$};


\end{tikzpicture}

